Optimizing Guided Traversal for Fast Learned Sparse Retrieval

Recent studies show that BM25-driven dynamic index skipping can greatly accelerate MaxScore-based document retrieval based on the learned sparse representation derived by DeepImpact. This paper investigates the effectiveness of such a traversal guidance strategy during top k retrieval when using other models such as SPLADE and uniCOIL, and finds that unconstrained BM25-driven skipping could have a visible relevance degradation when the BM25 model is not well aligned with a learned weight model or when retrieval depth k is small. This paper generalizes the previous work and optimizes the BM25 guided index traversal with a two-level pruning control scheme and model alignment for fast retrieval using a sparse representation. Although there can be a cost of increased latency, the proposed scheme is much faster than the original MaxScore method without BM25 guidance while retaining the relevance effectiveness. This paper analyzes the competitiveness of this two-level pruning scheme, and evaluates its tradeoff in ranking relevance and time efficiency when searching several test datasets.

==> table/block-stat.tex <==
\begin{table}[tpbh]
\scriptsize
    \centering
        %\caption{Relevance, time, and safeness of different design options on MS MARCO passage TREC19.\label{tab:abl}}
        \caption{ Characteristics of  design options on DL'19 passages}
        
        \setlength\tabcolsep{3pt}
        
\label{tab:options}
\resizebox{1.05\columnwidth}{!}{%
    \begin{tabular}{lrrrrr}
    \hline
    % & & \multicolumn{3}{c|}{Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
    %   &  &   & \bf{Overlap} & \bf{Loaded} &  \\
     \bf{Methods} & \bf{Time} & \bf{NDCG} & \bf{Overlap} & \bf{BLoad} & \bf{\# Eval}  \\ 
     \hline
    %  BM25-0 & 109 & 0.5501 & 26628 & 0.9524 & 344275 \\
     BM25-T5 & 75(166) & 0.579 & 48.36\% & 69.33\% & 157072 \\
     uniCOIL & 229(720) & 0.703 & 100\% & 95.21\% & 643842 \\
     uniCOIL, $F$=1.7 & 73(183) & 0.703 & 50.51\% & 74.22\% & 110221 \\
     \hline
     \multicolumn{6}{l}{uniCOIL/DTHS variations.  Default: $\alpha$=0.9, $\beta$=0.2, $F_s$=$F_f$=1; Independent view} \\
    %  UniCOIL (ST, Uniform) & 90 & 0.7163 & ?? & ?? & ?? \\
    %  UniCOIL- & & & & & & & & & & \\
     +$\alpha$=1 $\beta$=0;Single threshold  & 89(197) & 0.704 & 89.71\% & 69.00\% & 138439 \\
     +$\alpha$=1 $\beta$=0  & 84(172) & 0.704 & 89.45\%  & 68.99\% & 138353 \\
     +$\alpha$=1 $\beta$=0; Uniform & 185(390) & 0.703 & 99.99\% & 86.06\% & 521364 \\
     +$\alpha$=0.9 $\beta$=0 & 83(169) & 0.704 & 88.77\% & 68.99\% & 138283 \\
     \cline{1-1} 
     +$\alpha$=$\beta$=0.2 & 222(696) & 0.707 & 100\% & 88.93\% &  701961 \\
     +$\alpha$=0.9 $\beta$=0.2; Uniform & 170(333) & 0.707 & 99.99\% & 87.76\% & 787263 \\
     Default & 83(169) & 0.707 & 96.53\% & 69.00\% & 140719 \\
     +$F_s$=1.3 & 48(101) & 0.702 & 66.40\% & 47.31\% & 89683 \\
     +$F_s$=1.5 & 44(93) & 0.700 & 56.44\% & 42.54\% & 60485 \\
     +$F_s$=1.7 & 39(81) & 0.701 & 49.27\% & 39.53\% & 46351 \\
    %  UniCOIL (a, b) & 84 & 19289 & 0.6899 & 138283 \\
    %  UniCOIL (SepInd, B) & 13.3G & & & & & & & & & \\
    %  UniCOIL (SepInd, B+L) & 13.3G  & 0.4415 & 0.3239 & 0.9287 & 236 & 268 & 603 & & & \\
    %  UniCOIL (B Known thres) & 16.7G & 0.4735 & 0.3536 & 0.3536 & 191 & 211 & 455 & & & \\
    %  UniCOIL (SepInd, B Known thres) & & & & & & & & & & \\
     \hline
    \end{tabular}
    }
\end{table}


==> table/deepimpact-passage.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{DeepImpact-Passage (Intel NUC).\label{tab:p-di}}
    \begin{tabular}{c|ccc|c}
    \hline \hline
     Methods & NDCG & MRR & MAP & Time \\ \hline
     BM25 & 0.2965 & 0.1835 & 0.1805 & 17 \\
     DI & 0.4557 & 0.3392 & 0.3340 & 71 \\
     DI (BM25 guided) & 0.4556 & 0.3391 & 0.3339 & 57 \\
     DI (BM25 + DI guided) & 0.4236 & 0.3252 & 0.3201 & 46 \\
     DI (Index sep, BM25 guided) & & 0.3345 & & 38 \\
     DI (Index sep, BM25 + DI guided) & & 0.3235 & & 35 \\
     BM25 then DI (BM25 guided) & 0.4527 & 0.3385 & 0.3332 & 17+30 \\
     BM25 then DI (BM25 + DI guided) &  & 0.3246 & & 17+24 \\
     \hline \hline
    \end{tabular}
\end{table*}

==> table/overall.tex <==
\begin{table}[htbp]
%    \small
    \scriptsize

    \centering
%	\caption{Overall relevancy (MRR@10 and NDCG@10) and time comparison between baseline and proposed method. For time we report mean time and 95th percentile time in seconds: MRT(95T) .\label{tab:overall}}
        \caption{MRR(@10 for passages and @100 for documents), NDCG@10,  and mean/95th percentile time in milliseconds of different methods when $k$=1,000.}
\label{tab:overall}
        
        \resizebox{1.05\columnwidth}{!}{%
    \begin{tabular}{l|rr|rr|rr}
    \hline
     & \multicolumn{2}{c|}{\bf{Dev}} & \multicolumn{2}{c|}{\bf{TREC DL'19}} & \multicolumn{2}{c}{\bf{TREC DL'20}} \\
     \bf{Methods} & \bf{MRR} & \bf{Time} & \bf{NDCG} & \bf{Time} & \bf{NDCG} & \bf{Time}  \\ 
     
     \hline

     \multicolumn{7}{c}{\bf{MS MARCO Passages }} \\
     
     \hline
     BM25 & 0.172 & 17(42) & 0.425 & 52(140) & 0.453 & 54(157) \\
     BM25-T5 & 0.277 & 33(70) & 0.579 & 75(166) & 0.629 & 74(179) \\
     uniCOIL & 0.347 & 50(132) & 0.703 & 229(720) & 0.675 & 240(859) \\
     uniCOIL, $F$=1.7 & 0.346 & 30(74) & 0.703 & 73(183) & 0.675 &  75(234) \\
     uniCOIL, $F$=1.9 & 0.345 & \textbf{23(56)} & 0.695 & 55(124) & 0.672 & 60(172) \\
     DeepImpact & 0.328 & 71(166) & 0.695 & 235(751) & 0.628 & 243(855)  \\
     SPLADEv2 & 0.353 & 1373(2997) & 0.729 & 1513(3461) & 0.714 & 1400(3191) \\
     \hline
     uniCOIL/DTHS & 0.356 & 32(76) & 0.707 & 83(169) & 0.685 & 77(198)  \\
     + $F_s$=1.3,$F_f$=1 & 0.353 & 24(57) & 0.702 & \textbf{48(101)} & 0.675 & \textbf{46(110)} \\ 
     DeepImpact/DTHS & 0.344 & 45(96) & 0.710 & 108(302) & 0.675 & 111(261) \\
     SPLADEv2/DTHS & \textbf{0.362} & 896(1967) & \textbf{0.735} & 1059(2320) & \textbf{0.714} & 953(2067) \\

     \hline
     
     \multicolumn{7}{c}{\bf{MS MARCO Documents}} \\
     
     \hline
     
     BM25 & 0.203 & 165(351) & 0.446 & 171(373) & 0.451 & 169(422)  \\
     BM25-T5 & 0.303 & 205(435) & 0.559 & 179(374) & 0.561 & 174(408) \\
     uniCOIL & 0.353 & 494(1436) & 0.641 & 501(1461) & 0.601 & 512(2056) \\
    %  Unicoil thres 1.3 & & & 0.5882 & 287(771) & 0.6551 & 296(931) \\
    uniCOIL, $F$=1.5 & 0.352 & 207(525) & 0.641 & 203(531) & 0.601 & 203(609) \\
     uniCOIL, $F$=1.7 & 0.351 & 154(348) & 0.637 & 158(350) & 0.601 & 153(430) \\
    %  Unicoil thres 1.9 & & & 0.5670 & 132(277) & 0.6395 & 130(355) \\
     \hline
     uniCOIL/DTHS & \textbf{0.373} & 255(571) & \textbf{0.670} & 199(459) & \textbf{0.619} & 193(483) \\
     + $F_s$=1.3,$F_f$=1 & 0.371 & 173(385) & 0.670 & 127(282) & 0.619 & 125(304)  \\
     + $F_s$=1.5,$F_f$=1 & 0.367 & \textbf{130(284)} & 0.669 & \textbf{115(240)} & 0.619 & \textbf{113(269)}  \\ 
     \hline
    \end{tabular}
    }
\end{table}


==> table/overall23_bak.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ll|ll|ll|l|ll|ll|ll}
\hline
 & \multicolumn{6}{c|}{k=1000} &  & \multicolumn{6}{c}{k = 10} \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{2}{l|}{Dev} & \multicolumn{2}{l|}{DL19} & \multicolumn{2}{l|}{DL20} & \multicolumn{1}{l|}{} & \multicolumn{2}{l|}{Dev} & \multicolumn{2}{l|}{DL19} & \multicolumn{2}{l}{DL20} \\
\multicolumn{1}{l|}{Method} & MRR(recall) & \multicolumn{1}{l|}{mean time(99th)} & nDCG(recall) & \multicolumn{1}{l|}{mean time(99th)} & nDCG(recall) & \multicolumn{1}{l|}{mean time(99th)} & \multicolumn{1}{l|}{Method} & MRR(recall) & \multicolumn{1}{l|}{mean time(99th)} & nDCG(recall) & \multicolumn{1}{l|}{mean time(99th)} & nDCG(recall) & mean time(99th) \\ \hline
 & \multicolumn{13}{c}{MSMARCO Passage} \\ \hline
\multicolumn{1}{l|}{BM25-T5} & 0.2723(0.9348) & \multicolumn{1}{l|}{4.9(21.3)} & 0.6283(0.7704) & \multicolumn{1}{l|}{4.6(12)} & 0.6321(0.7598) & \multicolumn{1}{l|}{5.6(21.8)} & \multicolumn{1}{l|}{BM25-T5} & 0.2723(0.5319) & \multicolumn{1}{l|}{0.7(4.7)} & 0.6249(0.1611) & \multicolumn{1}{l|}{0.3(1.2)} & 0.6324(0.2218) & 0.5(4.1) \\
\multicolumn{1}{l|}{DeepImpact} & 0.3276(0.9474) & \multicolumn{1}{l|}{23.8(97)} & 0.6964(0.7623) & \multicolumn{1}{l|}{25.5(86.6)} & 0.6524(0.7534) & \multicolumn{1}{l|}{38.9(190)} & \multicolumn{1}{l|}{DeepImpact} & 0.3276(0.5844) & \multicolumn{1}{l|}{9.4(73.3)} & 0.6951(0.1698) & \multicolumn{1}{l|}{4.9(39)} & 0.6513(0.2035) & 7.8(48.9) \\
\multicolumn{1}{l|}{DeepImpact-GT} & 0.3276(0.9454) & \multicolumn{1}{l|}{5.1(21.1)} & 0.6964(0.7745) & \multicolumn{1}{l|}{4.9(13.6)} & 0.6527(0.7574) & \multicolumn{1}{l|}{5.8(22.6)} & \multicolumn{1}{l|}{DeepImpact-GT} & 0.3276(0.5805) & \multicolumn{1}{l|}{0.7(4.7)} & 0.6997(0.1698) & \multicolumn{1}{l|}{0.3(1.3)} & 0.6682(0.2194) & 0.5(4.3) \\
\multicolumn{1}{l|}{DeepImpact-GTI(50\%)} & 0.3413(0.9455) & \multicolumn{1}{l|}{5.2(21.7)} & 0.7072(0.7871) & \multicolumn{1}{l|}{4.7(13.3)} & 0.6854(0.7745) & \multicolumn{1}{l|}{5.7(22.8)} & \multicolumn{1}{l|}{DeepImpact-GTI(50\%)} & 0.3375(0.5866) & \multicolumn{1}{l|}{0.7(4.7)} & 0.6953(0.169) & \multicolumn{1}{l|}{0.3(1.3)} & 0.6846(0.2372) & 0.5(4.3) \\
\multicolumn{1}{l|}{DeepImpact-2GT-beta0\%} & 0.3276(0.9467) & \multicolumn{1}{l|}{7.4(32.8)} & 0.6964(0.7651) & \multicolumn{1}{l|}{7.9(25.4)} & 0.6524(0.7539) & \multicolumn{1}{l|}{9.1(25.9)} & \multicolumn{1}{l|}{DeepImpact-2GT-beta0\%} & 0.3276(0.584) & \multicolumn{1}{l|}{1.1(8.1)} & 0.6978(0.1703) & \multicolumn{1}{l|}{0.7(2.8)} & 0.656(0.2057) & 1.2(8.5) \\
\multicolumn{1}{l|}{DeepImpact-2GTI-beta0\%(50\%)} & 0.3414(0.9469) & \multicolumn{1}{l|}{7.4(33)} & 0.7072(0.7875) & \multicolumn{1}{l|}{7.8(25.6)} & 0.6854(0.7778) & \multicolumn{1}{l|}{9.1(26.3)} & \multicolumn{1}{l|}{DeepImpact-2GTI-beta0\%(50\%)} & 0.3405(0.5987) & \multicolumn{1}{l|}{1.1(8.1)} & 0.7065(0.1703) & \multicolumn{1}{l|}{0.7(2.8)} & 0.685(0.2361) & 1.2(8.5) \\
\multicolumn{1}{l|}{DeepImpact-2GTI-beta100\%(50\%)} & 0.3413(0.9455) & \multicolumn{1}{l|}{5.2(21.7)} & 0.7072(0.7871) & \multicolumn{1}{l|}{4.7(13.3)} & 0.6854(0.7745) & \multicolumn{1}{l|}{5.7(22.9)} & \multicolumn{1}{l|}{DeepImpact-2GTI-beta50\%(50\%)} & 0.3404(0.5986) & \multicolumn{1}{l|}{1(7)} & 0.7065(0.1703) & \multicolumn{1}{l|}{0.5(2.3)} & 0.685(0.2361) & 0.9(6.5) \\
\multicolumn{1}{l|}{UniCOIL} & 0.3516(0.9582) & \multicolumn{1}{l|}{35.3(196.7)} & 0.7027(0.7822) & \multicolumn{1}{l|}{38.6(286.3)} & 0.6746(0.7758) & \multicolumn{1}{l|}{42.8(225.5)} & \multicolumn{1}{l|}{DeepImpact-2GTI-beta90\%(50\%)} & 0.3395(0.5934) & \multicolumn{1}{l|}{0.7(5.1)} & 0.7045(0.1693) & \multicolumn{1}{l|}{0.4(1.6)} & 0.6882(0.2371) & 0.6(4.7) \\
\multicolumn{1}{l|}{UniCOIL-GT} & 0.3514(0.9458) & \multicolumn{1}{l|}{10.6(33.9)} & 0.7028(0.7857) & \multicolumn{1}{l|}{10.3(24.9)} & 0.6746(0.7741) & \multicolumn{1}{l|}{10.8(25.8)} & \multicolumn{1}{l|}{UniCOIL} & 0.3516(0.6168) & \multicolumn{1}{l|}{10.5(101.7)} & 0.7027(0.1761) & \multicolumn{1}{l|}{10.4(77.9)} & 0.6746(0.2346) & 14.2(99.5) \\
\multicolumn{1}{l|}{UniCOIL-GTI(10\%)} & 0.3552(0.9468) & \multicolumn{1}{l|}{10.6(33.2)} & 0.713(0.7917) & \multicolumn{1}{l|}{10.3(24.7)} & 0.6899(0.7857) & \multicolumn{1}{l|}{10.8(25.7)} & \multicolumn{1}{l|}{UniCOIL-GT} & 0.3347(0.5639) & \multicolumn{1}{l|}{2.1(11.2)} & 0.699(0.177) & \multicolumn{1}{l|}{1.7(10.2)} & 0.6769(0.2444) & 2.4(10.3) \\
\multicolumn{1}{l|}{UniCOIL-2GT-beta0\%} & 0.3516(0.9553) & \multicolumn{1}{l|}{16.6(68.3)} & 0.7037(0.7852) & \multicolumn{1}{l|}{15.5(45.7)} & 0.6746(0.7758) & \multicolumn{1}{l|}{16.4(45.9)} & \multicolumn{1}{l|}{UniCOIL-GTI(10\%)} & 0.3384(0.5678) & \multicolumn{1}{l|}{2.1(11.2)} & 0.6959(0.1733) & \multicolumn{1}{l|}{1.6(9.8)} & 0.6739(0.2422) & 2.4(10.2) \\
\multicolumn{1}{l|}{UniCOIL-2GTI-beta0\%(10\%)} & 0.3554(0.9566) & \multicolumn{1}{l|}{16.9(68.4)} & 0.713(0.7904) & \multicolumn{1}{l|}{15.5(46.1)} & 0.6899(0.7823) & \multicolumn{1}{l|}{16.5(46.9)} & \multicolumn{1}{l|}{UniCOIL-2GT-beta0\%} & 0.3514(0.6146) & \multicolumn{1}{l|}{3.3(18.9)} & 0.7033(0.1749) & \multicolumn{1}{l|}{2.4(16.4)} & 0.675(0.2375) & 3.4(14.7) \\
\multicolumn{1}{l|}{UniCOIL-2GTI-beta100\%(10\%)} & 0.3552(0.9468) & \multicolumn{1}{l|}{10.6(33.2)} & 0.7129(0.7917) & \multicolumn{1}{l|}{10.3(24.7)} & 0.6899(0.7857) & \multicolumn{1}{l|}{10.8(25.7)} & \multicolumn{1}{l|}{UniCOIL-2GT-beta30\%} & 0.3508(0.612) & \multicolumn{1}{l|}{2.6(14.8)} & 0.7027(0.1747) & \multicolumn{1}{l|}{1.9(12.4)} & 0.681(0.2396) & 2.8(11.7) \\
\multicolumn{1}{l|}{SpladeV2} & 0.3937(0.9832) & \multicolumn{1}{l|}{277.8(819)} & 0.7304(0.8286) & \multicolumn{1}{l|}{317.1(851.2)} & 0.729(0.8287) & \multicolumn{1}{l|}{306.7(896.7)} & \multicolumn{1}{l|}{UniCOIL-2GT-beta0\%(10\%)} & 0.355(0.6205) & \multicolumn{1}{l|}{3.3(19.2)} & 0.7135(0.1769) & \multicolumn{1}{l|}{2.4(16.4)} & 0.6891(0.2451) & 3.4(14.5) \\
\multicolumn{1}{l|}{SpladeV2-GT} & 0.2973(0.9648) & \multicolumn{1}{l|}{336.2(1048.2)} & 0.6636(0.803) & \multicolumn{1}{l|}{330.4(903.8)} & 0.6605(0.8072) & \multicolumn{1}{l|}{344.4(885.8)} & \multicolumn{1}{l|}{UniCOIL-2GT-beta30\%(10\%)} & 0.3548(0.6193) & \multicolumn{1}{l|}{2.6(14.3)} & 0.7135(0.1769) & \multicolumn{1}{l|}{1.9(12.4)} & 0.6891(0.2451) & 2.8(11.5) \\
SpladeV2-GTI(5\%) & 0.2961(0.9648) & 331.7(1059) & 0.6595(0.8025) & 318.2(932.8) & 0.6587(0.8066) & 333.2(892.1) & \\
\multicolumn{1}{l|}{SpladeV2-GT/c} & 0.3783(0.9713) & \multicolumn{1}{l|}{69.3(228.3)} & 0.7301(0.8266) & \multicolumn{1}{l|}{72.5(236.7)} & 0.7215(0.8244) & \multicolumn{1}{l|}{78.8(198.5)} & \multicolumn{1}{l|}{SpladeV2} & 0.3937(0.6801) & \multicolumn{1}{l|}{120.6(483)} & 0.7304(0.1776) & \multicolumn{1}{l|}{135(533.1)} & 0.729(0.2437) & 138(539.3) \\
\multicolumn{1}{l|}{SpladeV2-GT/s} & 0.3918(0.9603) & \multicolumn{1}{l|}{37.6(117.8)} & 0.7343(0.816) & \multicolumn{1}{l|}{37.1(135.8)} & 0.7259(0.8097) & \multicolumn{1}{l|}{40.2(108.1)} & \multicolumn{1}{l|}{SpladeV2-GT} & 0.272(0.5246) & \multicolumn{1}{l|}{120.8(437.9)} & 0.6379(0.1677) & \multicolumn{1}{l|}{129.8(481.6)} & 0.6106(0.2192) & 138.9(376.1) \\
 & & & & & & & SpladeV2-GTI(5\%) & 0.2687(0.5209) & 118.2(440.1) & 0.6352(0.1669) & 131.2(482.6) & 0.6083(0.2190) & 139.2(381.2) \\
\multicolumn{1}{l|}{SpladeV2-GTI/s(5\%)} & 0.3919(0.9592) & \multicolumn{1}{l|}{37.6(121.2)} & 0.7389(0.8171) & \multicolumn{1}{l|}{37.1(135.2)} & 0.729(0.8055) & \multicolumn{1}{l|}{40.3(107.9)} & \multicolumn{1}{l|}{SpladeV2-GT/c} & 0.3036(0.5544) & \multicolumn{1}{l|}{26.7(114)} & 0.6501(0.1572) & \multicolumn{1}{l|}{27.3(13.4)} & 0.6615(0.2345) & 30.8(125.3) \\
\multicolumn{1}{l|}{SpladeV2-2GT-beta0\%} & 0.3937(0.9832) & \multicolumn{1}{l|}{624.8(1647.8)} & 0.7304(0.8286) & \multicolumn{1}{l|}{833.1(2095.1)} & 0.729(0.8289) & \multicolumn{1}{l|}{738.4(1471.2)} & \multicolumn{1}{l|}{SpladeV2-GT/s} & 0.3457(0.576) & \multicolumn{1}{l|}{9.3(36.7)} & 0.6897(0.1632) & \multicolumn{1}{l|}{10.1(60.2)} & 0.7058(0.2455) & 11.7(59.5) \\
\multicolumn{1}{l|}{SpladeV2-2GT/c-beta0\%} & 0.3941(0.9828) & \multicolumn{1}{l|}{206.9(930.7)} & 0.7304(0.8288) & \multicolumn{1}{l|}{234.5(812)} & 0.729(0.8293) & \multicolumn{1}{l|}{223.1(642.4)} & \multicolumn{1}{l|}{SpladeV2-GTI/s(5\%)} & 0.3468(0.5774) & \multicolumn{1}{l|}{9.1(36.1)} & 0.6861(0.1624) & \multicolumn{1}{l|}{10.1(59.3)} & 0.7037(0.2438) & 11.5(58.6) \\
\multicolumn{1}{l|}{SpladeV2-2GT/s-beta0\%} & 0.3941(0.98) & \multicolumn{1}{l|}{110.5(475.6)} & 0.731(0.8139) & \multicolumn{1}{l|}{123.3(568.5)} & 0.729(0.8282) & \multicolumn{1}{l|}{133.3(512.6)} & \multicolumn{1}{l|}{SpladeV2-2GT-beta0\%} & 0.3937(0.6801) & \multicolumn{1}{l|}{442.4(1168.7)} & 0.7304(0.1776) & \multicolumn{1}{l|}{570.3(1404.7)} & 0.729(0.2437) & 503.6(1362) \\
\multicolumn{1}{l|}{SpladeV2-2GT/s-beta90\%} & 0.3933(0.9671) & \multicolumn{1}{l|}{42.9(143.6)} & 0.7323(0.8207) & \multicolumn{1}{l|}{42.2(161)} & 0.7279(0.8197) & \multicolumn{1}{l|}{45(119.9)} & \multicolumn{1}{l|}{SpladeV2-2GT/c-beta0\%} & 0.3937(0.6804) & \multicolumn{1}{l|}{69(361.4)} & 0.7324(0.1834) & \multicolumn{1}{l|}{72.7(440.3)} & 0.729(0.2437) & 75.3(316.9) \\
\multicolumn{1}{l|}{SpladeV2-2GTI/s-beta0\%(5\%)} & 0.3946(0.9799) & \multicolumn{1}{l|}{108.6(477.9)} & 0.7394(0.8209) & \multicolumn{1}{l|}{123(570.2)} & 0.7297(0.8339) & \multicolumn{1}{l|}{131.7(510.6)} & \multicolumn{1}{l|}{SpladeV2-2GT/s-beta0\%} & 0.3935(0.6786) & \multicolumn{1}{l|}{30.1(161.7)} & 0.7356(0.185) & \multicolumn{1}{l|}{31.9(299.4)} & 0.7237(0.2427) & 36.9(210.2) \\
\multicolumn{1}{l|}{SpladeV2-2GTI/s-beta90\%(5\%)} & 0.3937(0.9662) & \multicolumn{1}{l|}{43.1(143.6)} & 0.7394(0.8218) & \multicolumn{1}{l|}{42.1(161.2)} & 0.7306(0.8205) & \multicolumn{1}{l|}{45(121)} & \multicolumn{1}{l|}{SpladeV2-2GT/s-beta30\%} & 0.3924(0.6733) & \multicolumn{1}{l|}{22.8(115.7)} & 0.736(0.1831) & \multicolumn{1}{l|}{23.4(212.9)} & 0.7243(0.2431) & 26.1(137.2) \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{SpladeV2-2GTI/s-beta0\%(5\%)} & 0.3939(0.6812) & \multicolumn{1}{l|}{31.1(170.8)} & 0.7401(0.1846) & \multicolumn{1}{l|}{31.9(299.6)} & 0.7278(0.248) & 36.8(210.4) \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{SpladeV2-2GTI/s-beta30\%(5\%)} & 0.3934(0.6792) & \multicolumn{1}{l|}{22.7(115.7)} & 0.738(0.1837) & \multicolumn{1}{l|}{23.5(212.8)} & 0.7278(0.248) & 26.2(136.4) \\ \hline
 & \multicolumn{13}{c}{MSMARCO Documents} \\ \hline
\multicolumn{1}{l|}{BM25-T5} & 0.295(0.9197) & \multicolumn{1}{l|}{12.4(50)} & 0.5594(0.569) & \multicolumn{1}{l|}{15(72.7)} & 0.5742(0.7148) & \multicolumn{1}{l|}{15.7(42.7)} & \multicolumn{1}{l|}{BM25-T5} & 0.2716(0.4749) & \multicolumn{1}{l|}{2.7(13.9)} & 0.4246(0.0741) & \multicolumn{1}{l|}{3.6(53.6)} & 0.4463(0.1693) & 3.1(13) \\
\multicolumn{1}{l|}{UniCOIL} & 0.353(0.9426) & \multicolumn{1}{l|}{71(447.4)} & 0.6415(0.5864) & \multicolumn{1}{l|}{79.2(576.9)} & 0.6059(0.7502) & \multicolumn{1}{l|}{86(386.8)} & \multicolumn{1}{l|}{UniCOIL} & 0.3313(0.5638) & \multicolumn{1}{l|}{26(252.2)} & 0.5477(0.088) & \multicolumn{1}{l|}{28.1(227.2)} & 0.4996(0.192) & 27.3(143.2) \\
\multicolumn{1}{l|}{UniCOIL-GT} & 0.353(0.9361) & \multicolumn{1}{l|}{20.9(73.8)} & 0.6445(0.5842) & \multicolumn{1}{l|}{21.6(77.3)} & 0.6059(0.7444) & \multicolumn{1}{l|}{22.7(68.7)} & \multicolumn{1}{l|}{UniCOIL-GT} & 0.328(0.5455) & \multicolumn{1}{l|}{6.8(36.2)} & 0.5199(0.0779) & \multicolumn{1}{l|}{6.2(32.3)} & 0.4903(0.1871) & 7.1(39.7) \\
\multicolumn{1}{l|}{UniCOIL-GTI(10\%)} & 0.3639(0.9368) & \multicolumn{1}{l|}{20.6(72.9)} & 0.6581(0.592) & \multicolumn{1}{l|}{21.7(77.8)} & 0.6156(0.7445) & \multicolumn{1}{l|}{22.6(69.5)} & \multicolumn{1}{l|}{UniCOIL-GTI(10\%)} & 0.3334(0.5531) & \multicolumn{1}{l|}{6.9(36.6)} & 0.5223(0.0781) & \multicolumn{1}{l|}{5.9(31.4)} & 0.4905(0.1857) & 7.2(40.1) \\
\multicolumn{1}{l|}{UniCOIL-2GT-beta0\%} & 0.353(0.9411) & \multicolumn{1}{l|}{33(15)} & 0.6438(0.5842) & \multicolumn{1}{l|}{32.8(152.3)} & 0.6059(0.748) & \multicolumn{1}{l|}{36.1(134.3)} & \multicolumn{1}{l|}{UniCOIL-2GT-beta0\%} & 0.3312(0.5627) & \multicolumn{1}{l|}{10.4(56.6)} & 0.5482(0.0889) & \multicolumn{1}{l|}{9(82.5)} & 0.4996(0.192) & 10.6(54.3) \\
\multicolumn{1}{l|}{UniCOIL-2GTI-beta0\%(10\%)} & 0.3644(0.9422) & \multicolumn{1}{l|}{33.2(149.2)} & 0.6581(0.5932) & \multicolumn{1}{l|}{32.8(152.5)} & 0.6156(0.7477) & \multicolumn{1}{l|}{37.4(141.3)} & \multicolumn{1}{l|}{UniCOIL-2GT-beta50\%} & 0.3317(0.5909) & \multicolumn{1}{l|}{7.5(40.2)} & 0.545(0.0851) & \multicolumn{1}{l|}{6.5(46.6)} & 0.4992(0.1881) & 8.1(46.1) \\
\multicolumn{1}{l|}{UniCOIL-2GTI-beta100\%(10\%)} & 0.3639(0.9368) & \multicolumn{1}{l|}{20.6(73)} & 0.6581(0.592) & \multicolumn{1}{l|}{21.7(77.8)} & 0.6156(0.7445) & \multicolumn{1}{l|}{22.5(69.5)} & \multicolumn{1}{l|}{UniCOIL-2GTI-beta0\%(10\%)} & 0.3423(0.571) & \multicolumn{1}{l|}{10.2(56.4)} & 0.5486(0.0852) & \multicolumn{1}{l|}{8.9(82.3)} & 0.4998(0.1886) & 10.5(54) \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{UniCOIL-2GTI-beta50\%(10\%)} & 0.3418(0.5663) & \multicolumn{1}{l|}{7.4(40.4)} & 0.5453(0.0847) & \multicolumn{1}{l|}{6.5(46.6)} & 0.4997(0.1845) & 8.2(50.3) \\ \hline
\end{tabular}%
}
\end{table*}


==> table/recall.tex <==
\comments{
\begin{table}[tpbh]
    \scriptsize
    \centering
        \caption{Recall.\label{tab:recall}}
\label{tab:smallk}
    \begin{tabular}{l|rrr|rr}
    \hline 
    
    \hline
    %  & \multicolumn{2}{c|}{BM25-T5} &\multicolumn{2}{c|}{UniCOIL}& \multicolumn{2}{c|}{UniCOIL-1.7} & \multicolumn{2}{c}{DTHS} & \multicolumn{2}{c}{DTHS-1.3} \\
     \bf{k} & \bf{BM25-T5} & \bf{UniCOIL} & \bf{w/ TH 1.7} & \bf{UniCOIL (DTHS)} & \bf{w/ TH 1.3}  \\ \hline
     10 & 0.5135(17) & 0.6101(22) &  & 0.6003(14) & \\
     20 & 0.6135(18) & 0.7067(23) &  & 0.6959(15) & \\
     200 & 0.8484(25) & 0.8992(30) & & 0.8971(24) & \\
     1000 & 0.9363(34) & 0.9527(50) & & 0.9530(32) & \\
     \hline
     
     \hline
    \end{tabular}
\end{table}
}

\begin{table}[tpbh]
    % \scriptsize
    \centering

        %\caption{Performance in terms of  relevance MRR@10(Recall@k) and time MRT(95T) in seconds on MS MARCO pass. Dev set \label{tab:recall}}
        \caption{MRR(Recall@k) and  MRT(95T) on the Dev query set.\label{tab:recall}}
    \setlength\tabcolsep{3pt}
\label{tab:smallk}

\resizebox{1.04\columnwidth}{!}{%
    \begin{tabular}{l|rr|rr|rr|rr}
    \hline 
     & \multicolumn{2}{c|}{\bf k=10} &\multicolumn{2}{c|}{\bf k=20}& \multicolumn{2}{c|}{\bf k=200} & \multicolumn{2}{c}{\bf k=1000} \\
      & MRR(R.) & Time & MRR(R.) & Time & MRR(R.) & Time  & MRR(R.) & Time \\ \hline
      \multicolumn{9}{c}{\textbf{MS MARCO Passages Dev}} \\ \hline
     BM25-T5 & .277(.513) & 17(42) & .277(.614) & 18(44) & .277(.848) & 25(54) & .277(.936) & 33(70)  \\
    \hline 
     uniCOIL & .347(.610) & 22(52) & .347(.707) & 23(55) & .347(.899) & 30(71) & .347(.953) & 50(132) \\
      + $F$=1.1 & .346(.606) & 21(54) & .346(.702) & 22(55) & .347(.899) & 29(70) & .347(.953) & 44(110) \\
      + $F$=1.3 & .322(.549) & 17(46) & .336(.655) & 19(50) & .346(.886) & 27(68) & .347(.953) & 36(91) \\
      + $F$=1.7 & .236(.350) & 10(34) & .276(.462) & 12(39) & .340(.796) & 19(49) & .346(.919) & 30(74) \\
    \hline 
     DTHS & .350(.600) & 14(38) &  .353(.696) & 15(42) & .355(.897) & 24(63) & .356(.957) & 32(76) \\
      + $F_s$=1.01 & .348(.596) & 13(38) & .352(.694) & 15(40) & .355(.894) & 24(62) & .356(.957) & 31(74) \\
      + $F_s$=1.1 & .287(.448) & 11(35) & .313(.559) & 12(36) & .352(.833) & 19(54) & .355(.933) & 28(67) \\
      + $F_s$=1.3 & .217(.315) & 7(30) & .260(.420) & 9(34) & .339(.751) & 17(49) & .353(.897) & 24(57) \\

     \hline
     
           \multicolumn{9}{c}{\textbf{MS MARCO Documents Dev}} \\ \hline
     BM25-T5 & .291(.571) & 79(196) & .298(.673) & 87(208) & .303(.883) & 128(295) & .303(.925) & 205(435)  \\
    \hline 
     uniCOIL & .342(.640) & 213(587) & .349(.745) & 230(651) & .353(.918) & 334(1000) & .353(.943) & 494(1436) \\
      + $F$=1.1 & .331(.562) & 142(337) & .344(.669) & 159(387) & .353(.889) & 244(598) & .353(.943) & 330(816) \\
      + $F$=1.3 & .310(.506) & 100(210) & .332(.618) & 150(322) & .352(.878) & 183(435) & .353(.940) & 255(604) \\
      + $F$=1.5 & .255(.390) & 75(158) & .291(.504) & 89(173) & .347(.828) & 135(280) & .352(.924) & 199(459) \\
    \hline 
     DTHS & .349(.573) & 102(227) & .363(.678) & 114(257) & .373(.887) & 181(418) & .373(.942) & 255(571) \\
      + $F_s$=1.01 & .348(.571) & 99(220) & .362(.676) & 110(254) & .373(.887) & 176(407) & .373(.942) & 252(564) \\
      + $F_s$=1.1 & .333(.533) & 82(173) & .351(.640) & 96(219) & .371(.872) & 150(340) & .372(.937) & 221(496) \\
      + $F_s$=1.3 & .267(.397) & 62(129) & .303(.509) & 69(142) & .362(.819) & 111(236) & .371(.916) & 173(385) \\

     \hline
    \end{tabular}
    }
\end{table}


% \begin{table}[tpbh]
%     \scriptsize
%     \centering
%         \caption{Recall.\label{tab:recall}}
% \label{tab:smallk}
%     \begin{tabular}{c|cc|cc|cc}
%     \hline 
    
%     \hline
%      & \multicolumn{2}{c|}{BM25-T5} &\multicolumn{2}{c|}{UniCOIL}& \multicolumn{2}{c}{DTHS} \\
%      k & Recall(MRR) & Time & Recall(MRR) & Time & Recall(MRR) & Time  \\ \hline
%      10 & 0.5135(0.2587) & 17(42) & 0.6101(0.3466) & 22(52) & 0.6003(0.3445) & 14(38) \\
%      20 & 0.6135(0.2657) & 18(44) & 0.7067(0.3535) & 23(55) & 0.6959(0.3522) & 15(42) \\
%      200 & 0.8484(0.2707) & 25(54) & 0.8992(0.3576) & 30(71) & 0.8971(0.3574) & 24(63) \\
%      1000 & 0.9363(0.2709) & 34(74) & 0.9527(0.3577) & 50(132) & 0.9530(0.3605) & 32(76) \\

%      \hline
     
%      \hline
%     \end{tabular}
% \end{table}


==> table/unicoil-alpha.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage Dev Alpha Experiment.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Trec19 Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline

     Unicoil (B$_{T5}$), 0 & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 35 & 78 &  &  &  \\
     Unicoil (B$_{T5}$), 0.00005 (10\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 31 & 34 & 76 &  &  &  \\
     Unicoil (B$_{T5}$), 0.0001 (20\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 34 & 37 & 80 &  &  &  \\
     Unicoil (B$_{T5}$), 0.0004 (50\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 35 & 40 & 84 &  &  &  \\
     Unicoil (B$_{T5}$), 0.004 (90\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 41 & 47 & 111 &  &  &  \\
    
     \hline
     Unicoil (B$_{T5}$+L), 0 & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 34 & 77 &  &  &  \\
      Unicoil (B$_{T5}$+L), 0.00005 (10\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 30 & 32 & 73 &  &  &  \\
     Unicoil (B$_{T5}$+L), 0.0001 (20\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 34 & 37 & 79 &  &  &  \\
     Unicoil (B$_{T5}$+L), 0.0004 (50\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 35 & 40 & 84 &  &  &  \\
     Unicoil (B$_{T5}$+L), 0.004 (90\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 40 & 47 & 111 &  &  &  \\
    %  Unicoil (SepInd, B) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 106 & 115 & 253 &  &  &  \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 105 & 115 & 250 &  &  &  \\ 
    \hline
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}

==> table/unicoil-document.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Document.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 6.4G & 0.3389 & 0.2173 & 0.8651 & 149 & 167 & 355 & & & \\
     BM25+ & & & & & & & \\
     Unicoil & 6.9G & 0.4736 & 0.3535 & 0.9426 & 336 & 497 & 1456 & & & \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 10.3G & 0.4735 & 0.3536 & 0.9403 & 193 & 212 & 454 & & & \\
     Unicoil (B+L) & 10.3G & 0.4735 & 0.3536 & 0.9403 & 189 & 208 & 444 & & & \\
    %  Unicoil (SepInd, B) & 13.3G & & & & & & & & & \\
    %  Unicoil (SepInd, B+L) & 13.3G  & 0.4415 & 0.3239 & 0.9287 & 236 & 268 & 603 & & & \\
    %  Unicoil (B Known thres) & 16.7G & 0.4735 & 0.3536 & 0.3536 & 191 & 211 & 455 & & & \\
    %  Unicoil (SepInd, B Known thres) & & & & & & & & & & \\
     \hline \hline
    \end{tabular}
\end{table*}


% \begin{table*}[tpbh]
%     \centering
%         \caption{Unicoil-Document (Expanse).\label{tab:d-uni}}
%     \begin{tabular}{c|ccc|c}
%     \hline \hline
%      Methods & NDCG & MRR & MAP & Time \\ \hline
%      BM25 & 0.3469 & 0.2263 & 0.2263 & 222 \\
%      Unicoil & 0.4736 & 0.3535 & 0.3535 & 552 \\
%      Unicoil (BM25 guided) & 0.4735 & 0.3536 & 0.3536 & 290 \\
%      \hline \hline
%     \end{tabular}
% \end{table*}

==> table/unicoil-passage.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage Dev.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Dev Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 0.9G & 0.2972 & 0.1837 & 0.8374 & 16 & 19 & 46 & 14 & 17 & 42 \\
     BM25+0 & 1.4G & 0.2972 & 0.1837 & 0.8374 & 42 & 44 & 92 & & & \\
     BM25-T5 & 1.4G & 0.3954 & 0.2709 & 0.9363 & 33 & 35 & 74 &  &  &  \\ \hline
     Unicoil & 1.4G & 0.4735 & 0.3577 & 0.9527 & 44 & 52 & 135 & 43 & 50 & 132 \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 40 & 44 & 95 & 40 & 43 & 92 \\
     Unicoil (B$_{T5}$) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 35 & 78 &  &  &  \\
     Unicoil (B+L) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 38 & 42 & 88 & 38 & 41 & 88 \\
     Unicoil (B$_{T5}$+L) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 34 & 77   &  &  &  \\ 
     Unicoil (DSHS) & 2.0G & 0.4754 & 0.3605 & 0.9530 & 30 & 33 & 76 &  &  &  \\ \hline
    %  Unicoil (SepInd, B) & 2.1G & 0.4547 & 0.3389 & 0.9348 & 34 & 38 & 86 & 34 & 37 & 85 \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.4547 & 0.3389 & 0.9348 & 31 & 35 & 77 & 31 & 34 & 75 \\ \hline
     DeepImpact & 1.5G & 0.4557 & 0.3392 &  &  & 71 &  & & & \\
    %  DeepImpact- & & & & & & & & & & \\
     DeepImpact (B) & 2.2G & 0.4556 & 0.3391 &  & & 57 & & & & \\
     DeepImpact (B+L) & 2.2G & 0.4236 & 0.3252 &  & & 46 & & & & \\
    %  DeepImpact (SepInd, B) & 2.1G & & & & & & & & & \\
    %  DeepImpact (SepInd, B+L) & 2.1G & & 0.3235 &  & & 35 & & & & \\ 
    \hline
     SpladesV2 & 4.5G & 0.4618 & 0.3417 & 0.9613 & 49 & 60 & 151 & & & \\
    %  SpladesV2- & & & & & & & & & & \\
     SpladeV2 (B) & 6.7G & 0.4617 & 0.3417 & 0.9608 & 49 & 58 & 133 & & & \\
     SpladeV2 (B$_{T5}$) & 6.7G & 0.4613 & 0.3417 & 0.9581 & 43 & 50 & 108 & & & \\
     SpladeV2 (B+L) & 6.7G & 0.4617 & 0.3417 & 0.9608 & 48 & 57 & 130 & & & \\
     SpladeV2 (B$_{T5}$+L) & 6.7G & 0.4614 & 0.3417 & 0.9584 & 41 & 48 & 107 & & & \\
     SpladeV2 (DSHS) & 6.7G & 0.4623 & 0.3424 & 0.9589 & 42 & 49 & 110 & & & \\
    %  SpladeV2 (SepInd, B) & 2.1G & & & & & & & & & \\
    %  SpladeV2 (SepInd, B+L) & 2.1G & &  &  & & & & & & \\ \hline
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}

\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage TREC19.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Trec19 Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 0.9G & 0.5501 & 0.7396 & 0.7081 & 54 & 63 & 144 & 53 & 52 & 140 \\
    %  BM25+0 & 1.4G & 0.6653 & 0.8857 & 0.7586 & 102 & 109 & 243 &  &  &  \\
     BM25-T5 & 1.4G & 0.6653 & 0.8857 & 0.7586 & 77 & 78 & 169 &  &  &  \\ \hline
     Unicoil & 1.4G & 0.7163 & 0.9767 & 0.7822 & 148 & 230 & 722 & 135 & 229 & 720 \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 2.0G & 0.7171 & 0.9767 & 0.7839 & 112 & 113 & 233 & 112 & 113 & 230 \\
     Unicoil (B$_{T5}$) & 2.0G & 0.7171 & 0.9767 & 0.7839 & 91 & 89 & 197 &  &  &  \\
     Unicoil (B+L) & 2.0G & 0.7169 & 0.9767 & 0.7836 & 109 & 108 & 222 & 107 & 107 & 221 \\
     Unicoil (B$_{T5}$+L) & 2.0G & 0.7169 & 0.9767 & 0.7836 & 86 & 84 & 172 &  &  &  \\
     Unicoil (DSHS) & 2.0G & 0.7194 & 0.9767 & 0.7854 & 86 & 84 & 170 & 85 & 83 & 169 \\
    %  Unicoil (SepInd, B) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 106 & 115 & 253 &  &  &  \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 105 & 115 & 250 &  &  &  \\ 
    \hline
    
    DeepImpact & 1.5G & 0. & 0. & 0. &  &  &  &  &  &  \\
    DeepImpact (B) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     
     \hline
     
     SpladeV2 & 4.5G & 0.7346 & 0.9612 & 0.8214 & 119 & 159 & 416 &  &  &  \\
    SpladeV2 (B) & 6.7G & 0.7346 & 0.9612 & 0.8217 & 85 & 112 & 260 &  &  &  \\
     SpladeV2 (B$_{T5}$) & 6.7G & 0.7354 & 0.9612 & 0.8245 & 90 & 109 & 249 &  &  &  \\
     SpladeV2 (B+L) & 6.7G & 0.7343 & 0.9612 & 0.8213 & 82 & 107 & 249 &  &  &  \\
     SpladeV2 (B$_{T5}$+L) & 6.7G & 0.7354 & 0.9612 & 0.8244 & 72 & 89 & 201 &  &  &  \\
     SpladeV2 (DSHS) & 6.7G & 0.7379 & 0.9612 & 0.8256 & 71 & 88 & 200 &  &  &  \\
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}

\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage TREC20.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Trec20 Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 0.9G & 0.5156 & 0.8286 & 0.6455 & 47 & 56 & 161 & 43 & 54 & 157 \\
    %  BM25+0 & 1.4G & 0. & 0. & 0. &  &  &  &  &  &  \\
     BM25-T5 & 1.4G & 0.6531 & 0.9444 & 0.7564 & 67 & 75 & 183 &  &  &  \\ \hline
     Unicoil & 1.4G & 0.6937 & 0.9338 & 0.7758 & 142 & 247 & 896 & 136 & 240 & 895 \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 2.0G & 0.6940 & 0.9338 & 0.7765 & 93 & 105 & 273 & 95 & 108 & 251 \\
     Unicoil (B$_{T5}$) & 2.0G & 0.6932 & 0.9338 & 0.7732 & 74 & 80 & 202 &  &  &  \\
     Unicoil (B+L) & 2.0G & 0.6940 & 0.9338 & 0.7765 & 88 & 100 & 243 & 86 & 98 & 240 \\
     Unicoil (B$_{T5}$+L) & 2.0G & 0.6930 & 0.9338 & 0.7729 & 74 & 79 & 200 &  &  &  \\
     Unicoil (DSHS) & 2.0G & 0.6972 & 0.9369 & 0.7760 & 74 & 78 & 198 &  &  &  \\
    %  Unicoil (SepInd, B) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 106 & 115 & 253 &  &  &  \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 105 & 115 & 250 &  &  &  \\ 
    \hline
    
    DeepImpact & 1.5G & 0. & 0. & 0. &  &  &  &  &  &  \\
    DeepImpact (B) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     
     \hline
     
     SpladeV2 & 4.5G & 0.7068 & 0.9374 & 0.7969 & 105 & 155 & 464 &  &  &  \\
    SpladeV2 (B) & 6.7G & 0.7042 & 0.9374 & 0.7922 & 80 & 108 & 320 &  &  &  \\
     SpladeV2 (B$_{T5}$) & 6.7G & 0.7049 & 0.9374 & 0.7955 & 82 & 107 & 297 &  &  &  \\
     SpladeV2 (B+L) & 6.7G & 0.7042 & 0.9374 & 0.7922 & 77 & 104 & 315 &  &  &  \\
     SpladeV2 (B$_{T5}$+L) & 6.7G & 0.7050 & 0.9374 & 0.7957 & 65 & 86 & 245 &  &  &  \\
     SpladeV2 (DSHS) & 6.7G & 0.7065 & 0.9374 & 0.7982 & 66 & 86 & 245 &  &  & \\
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}
